Robust Phase Retrieval by Alternating Minimization

We consider a least absolute deviation (LAD) approach to the robust phase retrieval problem that aims to recover a signal from its absolute measurements corrupted with sparse noise. To solve the resulting non-convex optimization problem, we propose a robust alternating minimization (Robust-AM) derived as an unconstrained Gauss-Newton method. To solve the inner optimization arising in each step of Robust-AM, we adopt two computationally efficient methods for linear programs. We provide a non-asymptotic convergence analysis of these practical algorithms for Robust-AM under the standard Gaussian measurement assumption. These algorithms, when suitably initialized, are guaranteed to converge linearly to the ground truth at an order-optimal sample complexity with high probability while the support of sparse noise is arbitrarily fixed and the sparsity level is no larger than $1/4$. Additionally, through comprehensive numerical experiments on synthetic and image datasets, we show that Robust-AM outperforms existing methods for robust phase retrieval offering comparable theoretical performance

==> macros.tex <==
\RequirePackage{mathrsfs}
% \RequirePackage{xcolor}
% \PassOptionsToPackage{dvipsnames}{xcolor}
\RequirePackage{tcolorbox}
\RequirePackage{bm}
\RequirePackage[bb=boondox]{mathalfa}

\global\long\def\mb#1{\hm{#1}}
\global\long\def\mbb#1{\mathbb{#1}}
\global\long\def\mc#1{\mathcal{#1}}
\global\long\def\mcc#1{\mathscr{#1}}
\global\long\def\mr#1{\mathrm{#1}}
\global\long\def\msf#1{\mathsf{#1}}
\global\long\def\mfk#1{\mathfrak{#1}}
\global\long\def\E{\mbb E}
\global\long\def\P{\mbb P}
\global\long\def\var{\ensuremath{\mr{var}}}
\global\long\def\T{{\scriptscriptstyle{\textup{\textsf{T}}}}} %{{\scalebox{0.55}{\ensuremath{\msf T}}}}
\global\long\def\F{{\scriptstyle{\textup{F}}}} %{{\scalebox{0.55}{\ensuremath{\mr F}}}}
\global\long\def\d{\ensuremath{\mr d}}
\global\long\def\tr{\ensuremath{\mr{tr}}}
\global\long\def\supp{\ensuremath{\,\mr{supp}}}
\global\long\def\sgn{\ensuremath{\,\mr{sgn}}}
\global\long\def\argmax{\operatorname*{argmax}}
\global\long\def\argmin{\operatorname*{argmin}}
\global\long\def\defeq{\stackrel{\textup{\tiny def}}{=}}
\global\long\def\bbone{\mbb 1}
\global\long\def\norm#1{{\left\lVert #1\right\rVert }}
\global\long\def\inp#1{{\langle#1\rangle}}%
\global\long\def\conj#1{\overline{#1}}

\renewcommand{\hat}[1]{\widehat{#1}}
\renewcommand{\tilde}[1]{\widetilde{#1}}
% \DeclareMathOperator{\Tr}{Tr}



\newcommand*{\bmx}[1]{%
{
\begin{bmatrix}
	#1
\end{bmatrix}
%
}}

\RequirePackage{tcolorbox}
\tcbuselibrary{skins, breakable}
\newcommand*{\thmbox}[1]{
	\begin{tcolorbox}[	breakable, 
						enhanced, 
						frame hidden,
						colback=Dandelion!40!Yellow!20!White] %green!60!blue!10!white
		#1
	\end{tcolorbox}

}
